OMG-ATTACK: Self-Supervised On-Manifold Generation of Transferable Evasion Attacks

Evasion Attacks (EA) are used to test the robustness of trained neural networks by distorting input data to misguide the model into incorrect classifications. Creating these attacks is a challenging task, especially with the ever-increasing complexity of models and datasets. In this work, we introduce a self-supervised, computationally economical method for generating adversarial examples, designed for the unseen black-box setting. Adapting techniques from representation learning, our method generates on-manifold EAs that are encouraged to resemble the data distribution. These attacks are comparable in effectiveness compared to the state-of-the-art when attacking the model trained on, but are significantly more effective when attacking unseen models, as the attacks are more related to the data rather than the model itself. Our experiments consistently demonstrate the method is effective across various models, unseen data categories, and even defended models, suggesting a significant role for on-manifold EAs when targeting unseen models.

==> sections/background.tex <==
\section{Background}

%Adversarial attacks were first introduced in 2004 by \cite{Dalvi2004AdversarialC}, and gained more attention in 2014 after the work by \cite{Goodfellow2014ExplainingAH}. They showed that it is possible to create images that are almost indistinguishable from natural images but can be misclassified by a neural network. Studying adversarial attacks \cite{chakraborty2021survey,akhtar2018threat} is important because it helps improve the security and reliability of deep learning models. Adversarial attacks can potentially cause serious harm in real-world scenarios, such as when deep learning models are used for critical applications like self-driving cars, medical diagnosis, and financial transactions. Understanding how adversarial attacks work and developing effective defense mechanisms can help ensure the robustness and trustworthiness of deep learning models, making them more reliable and safer for use in these critical applications. Consequently, these attacks can be used to evaluate the robustness of a model and identify vulnerabilities. 

\subsection{Evasion Attacks}
Evasion attack methods can be grouped by several traits such as the amount of available information, the adversary's goal, or the perturbation size, each trait should be considered when an attack is analyzed.

\paragraph{White-box vs. Black-box} 
The availability of information about the threat model. In a white-box attack, the attacker has full knowledge of the model's architecture, parameters, and training data, allowing them to carefully craft the input perturbations to deceive the model \cite{madry2017towardsdeeplearning,MoosaviDezfooli2015DeepFoolAS}. For Example, FGSM \cite{Goodfellow2014ExplainingAH}  uses a direct optimization on the input to maximize its loss, and hence fool the threat model. 

\begin{align}
x^{adv} = x + \epsilon \cdot \operatorname{sign}(\nabla_{x} J(\theta, x, y)) \
\end{align}

where $x^{adv}$ is the adversarial example, $x$ is the original example, $\epsilon$ is the magnitude of the perturbation in $L_{\infty}$ norm, $J(\theta, x, y)$ is the loss function with parameters $\theta$ and target label $y$, and $\operatorname{sign}(\nabla_{x} J(\theta, x, y))$ is the sign of the gradient with respect to the input $x$.
Here the availability of the gradients allows for precise changes that will directly affect the loss function and therefore the prediction. 
%See Fig \ref{fig:fgsm_panda}


% \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.6\textwidth]{omg-attack-arow23/figures/fgsm_panda_image.png}
%  \caption{FGSM perturbation example.}
%  \label{fig:fgsm_panda}
% \end{figure}



On the other hand, in a black-box attack, the attacker has no knowledge of the model's internal workings and must rely on input-output observations to craft perturbations. so they need to exploit some other information in order to create these perturbations. some approaches include learning a distilled model of the black-box model.

Black-box attacks can be roughly divided into transfer-based attacks and query-based attacks. Transfer-based attacks adopt the gradient of a surrogate white-box model to generate adversarial examples, which are probable to fool the black-box model due to the transferability \cite{mifgsm,Liu2016DelvingIT,Papernot2016PracticalBA}.

Query-based attacks estimate the gradient by the zeroth-order optimization methods when the loss values could be accessed through queries. It was shown that it is possible to estimate the gradient at each coordinate and use it as a basis for attacks \cite{chen2017zoozerothorder}.


%\paragraph{Targeted vs Untargeted} 
%\adi{I don't think we need this, all of our attacks are untargeted}
%The goal of the adversary. In a targeted attack, the attacker specifically crafts the perturbations over the input data $\mathbf{x}'$ with the aim of causing the model to make a specific, targeted mistake $c_{target} = f(\mathbf{x}') \neq f(\mathbf{x}) = c_{original}$. On the other hand, in an untargeted attack, the attacker's goal is simply to cause the model to make any incorrect prediction without specifying a particular target class. Namely to generate an example $\mathbf{x}'$ such that $f(\mathbf{x}') \neq f(\mathbf{x})$, with no specific target class for $f(\mathbf{x}')$.


\paragraph{Perturbation Size}
The magnitude of the perturbation applied to the original input is crucial in the creation of adversarial examples. Most works place a limit on the size of the perturbation, measured by $L_p$ norms, for several reasons. Firstly, it serves as a metric for the similarity between the generated example and the original input. Secondly, it can be used to compare between methods and is commonly referred to as \textit{``attack strength''}. Two methods with the same perturbation size can affect the input differently, and the method that harms the model more is considered the better attack. Additionally, keeping the perturbation size small can make the adversarial example indistinguishable from the original example to the human eye, resulting in visually imperceptible attacks \cite{qian2020visuallyimperceptible}. Some adversarial methods, however, rely on operators that cannot be measured by distance metrics \cite{baluja2017adversarial}, while others use alternative methods to measure similarity, such as user studies \cite{duan2020adversarialcamouflage}.
\adi{need to refer to this as the budget, since this is what we use for the rest of the paper}

\subsection{Defenses Against Evasion Attacks}
To defend against an evasion attack is to reduce the effectiveness of adversarial examples against the threat model. different methods target different stages of the threat model, modifying the network, training data, or inference process. 
Currently, various techniques are employed to defend against adversarial attacks in machine learning models. These techniques can be broadly categorized into three groups: 

\paragraph{Adversarial Training}
The first group of methods focuses on making the model representations more robust to the adversarial examples. The most straightforward way to achieve this is simply by incorporating adversarial examples into the training process as in \cite{Goodfellow2014ExplainingAH,Addepalli2022ScalingAT,Pang2020BagOT}. This can be achieved by adding a component to the loss function that specifically penalizes the model for misclassifying adversarial examples:
\[ \mathbf{J}(\Theta, x, y) = \alpha \mathbf{J}(\Theta, x, y) + (1 - \alpha)\mathbf{J}(\Theta, x_{adv},y) \]

\paragraph{Limiting Sensitivity to Perturbations}
The second group of methods aims to limit the impact of adversarial perturbations on the activations of hidden layers by introducing different activation functions \cite{Xiao2019EnhancingAD} or input manipulations such as blurring, quantization \cite{lin2019defensive}, or resizing. These methods can effectively reduce the model's vulnerability to adversarial attacks. Still, they may also introduce additional computational overhead and may not be suitable for all types of models.

\paragraph{Adversarial Examples Detection }
The third category of methods focuses on detecting adversarial examples and treating them differently. This can be accomplished using various techniques, such as adversarial detection networks, which train a separate model to distinguish between normal and adversarial examples. These methods can be effective in detecting and reducing the impact of adversarial attacks, but they may require additional computational resources and may not be able to detect all forms of adversarial examples. Some works rely on statistical inference, making different assumptions about data distributions or activation distributions \cite{saha2019attackagnosticstatistical,Metzen2017OnDA,Ma2019NICDA}.

Overall, defending against adversarial attacks remains a challenging task, and the effectiveness of a particular defense method depends on the specific type of attack and the model architecture. A combination of multiple defense methods may be necessary to achieve robustness against a wide range of adversarial attacks.


% \subsection{Generative Models}
% \adi{this subsection is not needed IMO}
% Generative Models try to produce synthetic data that is in agreement with the original data distribution and to do so they try to learn and model the distribution of the original dataset. There are various approaches as to how to model the original data distribution and how to sample it into new synthetic data.

%  \paragraph{Generative Adversarial Networks (GANs) \cite{goodfellow2020generative}}  pose the training process as a game between two separate networks: a generator network and a second discriminative network that tries to classify samples as either coming from the true distribution $p(x)$ or the model distribution $p(x)'$. Every time the discriminator notices a difference between the two distributions the generator adjusts its parameters slightly to make it go away, until at the end (in theory) the generator exactly reproduces the true data distribution and the discriminator is guessing at random, unable to find a difference.

%  \paragraph{Variational Auto Encoders (VAEs) \cite{welling2014auto}} use a neural network encoder to map input data into a latent space, where the distribution of the data is modeled using a multivariate Gaussian distribution. A decoder network is then used to generate new data from this latent space. The goal is to train the network to minimize the reconstruction error between the original data and the generated data while also regularizing the latent space distribution to match a prior distribution, typically a standard normal distribution.

% \paragraph{Autoregressive models} such as PixelRNN \cite{https://doi.org/10.48550/arxiv.1601.06759}, is a type of generative model that models the conditional probability distribution of each feature in a sequence given its previous features. The name "autoregressive" comes from the fact that each feature is regressed on its own previous values.


% Generative models have gained significant attention in recent years due to their wide range of applications. One example is the use of generative models in image editing applications, such as Snapchat and Instagram, to create filters that generate a new avatar based on user photos. NVIDIA has also utilized generative models for realistic simulation environments, such as in their DRIVE Sim platform for self-driving car training.

% In the field of natural language processing, generative models have also shown great potential, such as OpenAI's GPT series of models \cite{Brown2020LanguageMA,Ouyang2022TrainingLM}, which have achieved state-of-the-art results in various NLP tasks including language modeling, text generation, summarization, and question answering. Additionally, generative models have also been used for music generation, video prediction, and speech synthesis applications.


% \subsection{Self-Supervised Representation Learning}
% \adi{this subsection is not needed IMO}
% Self-supervised representation learning is a type of machine learning that involves training a model to learn a representation of data without the use of explicit labels. In self-supervised learning, the model is provided with a dataset and a set of pre-defined tasks or objectives, and it must learn to perform these tasks using only the information present in the dataset.

% Self-supervised learning obtains supervisory signals from the data itself, often leveraging the underlying structure of the data. The general technique of self-supervised learning is to predict any unobserved or hidden part (or property) of the input from any observed or unhidden part of the input. 
% For example, as is common in NLP, we can hide part of a sentence and predict the hidden words from the remaining words \cite{devlin2018bert}. We can also predict past or future frames in an audio signal (hidden data) from current ones (observed data), or complete an image with missing data. For example, \cite{Baevski2022data2vecAG} shows that the mask out strategy works also for multimodal representation learning.

% Since self-supervised learning uses the structure of the data itself, it can make use of a variety of supervisory signals across co-occurring modalities (e.g., video and audio) and across large data sets — all without relying on labels. For example in \cite{caron2021emerging,grill2020bootstrap,krishnan2021eli5asimple} common image processing augmentations to were used to create different versions of the same image, and requested that the models will result in similar representations or activations for the different inputs.



==> sections/experimental_setup.tex <==
\section{Experiments} 

The goal of our experiments is to assess the efficacy of our model in generating adversarial examples. To that end, we evaluate our method by conducting experiments in various settings, including the white-box setting,  transferability to black-box models and architectures, including defended target models and  transferability of attacks to unseen data classes at train time.

% \paragraph{Datasets \& Models}
% We evaluate our pipeline on three datasets from different domains and target models at different scales and architectures on the classification task. The datasets are presented in \ref{tab:datasets}.%, and models in \ref{tab:models}.

%For each dataset, We chose a pretrained target model to attack, and since the resolutions differ, we also paired a discriminator for every dataset. 


\subsection{Experimental Setup}
\paragraph{Datasets \& Models}
We evaluate our pipeline on three datasets from different domains, using target models of various scales and architectures for the classification task. The datasets used are presented in Table \ref{tab:datasets}.

\input{tables/exp_datasets_tbl}

For each dataset, we train \ofirmodel{} (comprising a discriminator and generator) against a pre-trained model on the classification task of that particular dataset. For the \mnist{} dataset, we use the same target network architecture based on a Convolutional Neural Network (CNN) as used by Carlini \& Wagner \cite{Carlini2016TowardsET} (denoted as MNIST-CNN), which has 1.2M parameters. For the German Traffic Sign Recognition Benchmark (\traffic{}), we use a CNN with three Spatial Transformers \cite{Garca2018DeepNN}, which achieves over 99\% accuracy on this dataset (denoted as TS-CNN-STN) with 855K parameters. Lastly, for the Caltech Birds (\birds{}) dataset, we use the popular \resnet{} model \cite{He2015DeepRL} with 11.3M parameters (denoted as CUB-\resnet{}). 

As these models were used in training, we evaluate attacks on them under \textit{white-box} settings, where we have full access to the model parameters.

Under the \textit{black-box} settings, we use additional models to examine transferability. We leverage the \ofirmodel{} models trained under the white-box setting on each dataset separately and generate attacks for other unseen models. For MNIST, we use two models proposed by \cite{Tramr2017EnsembleAT} (denoted as \mnist{}-TR1 and \mnist{}-TR2) as well as a larger-scale \resnet{} trained on \mnist{}. For \traffic{}, we validate against a larger-scale \resnetf{}. Lastly, for the \birds{} dataset, we evaluate against a larger-scale \resnetf{} and \wideresnet{}.

further details about the models including the hyperparameters used are provided in the Appendix ~\ref{apx:exp_settings}

% \begin{table}[ht]
% \small
% \centering
% \begin{tabularx}{\columnwidth}{XXX}
% \toprule
% \textbf{Dataset} & \textbf{Target Model} & \textbf{\#Parameters}  \\ 
% \midrule
% MNIST & Model C & 1.2M \\ 
% GTSRB & STN-CNN & 855K \\ 
% CUB-200 & ResNet-18 & 11.3M \\ 
% \bottomrule
% \end{tabularx}
% \setlength{\abovecaptionskip}{10pt}
% \caption{Pretrained models used as targets for the training of \ofirmodel{} and AdvGAN, as well as for generating attacks in the white box baseline scenarios. The number of parameters for each model indicates the model's complexity. The target models are trained for the classification task specific to each dataset.}
% \label{tab:models}
% \end{table}


% \paragraph{Baselines}
% In order to compare the performance of our model with other methods, we chose to use several baseline models for benchmarking. 

% \begin{enumerate}
%     \item Fast Gradient Sign Method (FGSM) \cite{Goodfellow2014ExplainingAH}. This method is widely used in adversarial attack research due to its simplicity and effectiveness.

%     \item Projected Gradient Decent (PGD) \cite{Madry2017TowardsDL}. PGD is an iterative attack method used in adversarial research. Unlike FGSM, PGD takes multiple steps and has an epsilon ball constraint to generate more robust adversarial examples.

%     \item Momentum Iterative Fast Gradient Sign Method (MI-FGSM)  \cite{Dong2017BoostingAA}. MI-FGSM is an advanced adversarial attack method that aims to improve transferability by combines the ideas of FGSM and momentum. It takes multiple steps with a momentum term to generate more effective and robust adversarial examples. 

%     \item Variance-Tuning Momentum Iterative Fast Gradient Sign Method (VMI-FGSM)  \cite{Wang2021EnhancingTT}. VMI-FGSM is a further extension of the MI-FGSM method. It includes a variance term to adaptively adjust the step size during the iterative process. VMI-FGSM is considered one of the most powerful adversarial attack methods available, capable of generating highly effective and robust adversarial examples.

%     \item AdvGAN \cite{xiao2018generating}. This is a generative network-based method for generating adversarial examples and operates in the same domain as our model. 
% \end{enumerate}

\paragraph{Baselines}
To comprehensively evaluate the effectiveness of our proposed model, we draw comparisons with an array of adversarial attack methods that span from simple, yet effective strategies to more complex and robust methods. This range of baselines allows us to benchmark our model against both traditional and state-of-the-art techniques.

\begin{enumerate}
    \item \textbf{Fast Gradient Sign Method (\fgsm)} \cite{Goodfellow2014ExplainingAH}: The method utilizes the gradients of the loss function with respect to the input data to create adversarial perturbations.
    
    \item \textbf{Projected Gradient Descent (\pgd)} \cite{Madry2017TowardsDL}: Building upon FGSM, PGD introduces iterative attacks to adversarial research. Unlike FGSM, PGD applies the perturbations multiple times within an epsilon ball, offering more potent adversarial examples with enhanced robustness.

    \item \textbf{Momentum Iterative Fast Gradient Sign Method (\mifgsm)}  \cite{Dong2017BoostingAA}: This advanced adversarial attack method infuses momentum into the iterative FGSM process. The momentum term allows the method to maintain the direction of gradient update across iterations, thereby enhancing both the effectiveness and robustness of the generated adversarial examples.

    \item \textbf{Variance-Tuning Momentum Iterative Fast Gradient Sign Method (\vmifgsm)}  \cite{Wang2021EnhancingTT}: As an extension to MI-FGSM, VMI-FGSM introduces a variance term to dynamically adjust the step size throughout the iterative process. This adaptive approach yields highly potent adversarial examples, thus placing VMI-FGSM among the most powerful adversarial attack methods to date.

    \item \textbf{\advgan} \cite{xiao2018generating}: a generative adversarial network-based method for creating adversarial examples. It employs a similar domain of operation as our proposed model, thus providing a pertinent benchmark for comparison.
\end{enumerate}



% \paragraph{Evaluation Metrics}
% To evaluate the effectiveness of our adversarial augmentations, we use the following metrics:

% \begin{itemize}
%     \item \textbf{Attack Success Rate (ASR):} ASR measures the effectiveness of an adversarial attack. It is defined as the fraction of adversarial examples that successfully cause the target model to change its prediction. Mathematically, the ASR can be expressed as:

%     $$ASR = \frac{|\{X_{adv} | f(X) \neq f(X_{adv})\}|}{|\{X_{adv}\}|}$$
    
%     where $X_{adv}$ is an adversarial example generated from $X$. ASR is typically expressed as a percentage, with higher values indicating a more effective attack.
    
%     \item \textbf{ASR under Defense:} Measuring the ASR on models that are defended against adversarial examples demonstrates the robustness of the adversarial example, as regular models are usually vulnerable to adversarial attacks. The ASR under defense provides an evaluation metric that accounts for the attack's effectiveness against models designed to be robust to adversarial examples. \adi{elaborate and add citations. see background}
% \end{itemize}

\paragraph{Evaluation Metrics}
 We use the Attack Success Rate (ASR) to evaluate the effectiveness of our adversarial augmentations. ASR is defined as the fraction of adversarial examples that successfully cause the target model to change its prediction. Formally, 
 
 $$ASR = \frac{|\{X_{adv} | f(X) \neq f(X_{adv})\}|}{|\{X_{adv}\}|}$$
    
where $X_{adv}$ is an adversarial example generated from $X$. ASR is typically expressed as a percentage, with higher values indicating a more effective attack.

\input{tables/res_white_box}
\input{tables/res_unseen_models}

\paragraph{Budget Selection} We manually select an appropriate budget for each dataset and match it against all baselines. We acknowledge that this selection is not entirely comparable as the methods operate under different $L_p$ norms, and address this challenge in the limitation section. We set the budget for \mnist{} to be 0.3, for the \traffic{} we set 0.015, and for \birds{} 0.025. Additional details and ablation is provided in section ~\ref{sec:ablations}.

% \paragraph{Implementation details}
% All \ofirmodel{} configurations were trained with different datasets' specific parameters, which we describe fully in the appendix \ref{apx:exp_settings}. 




==> tables/apx_birds_examples.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/birds_showcase-11.png}
  \caption{Evasion Attacks on \birds{} dataset representative. On the left we have the original image, then the EAs using FGSM, then the diff. on the right side, we have the same paradigm for EAs generated using \ofirmodel{} model.}
  \label{fig:birds_showcase3}
\end{figure*}


==> tables/apx_hyperprameters.tex <==
\begin{table}[ht]
\centering
\begin{tabularx}{\linewidth}{Xr}
\toprule
\textbf{Module} & \textbf{\# Parameters} \\ 
\midrule
Generator & 1.8M \\
Discriminator & 1.6M \\
\mnisttgt{} & 694K \\ 
\mnisttra{} & 629K \\ 
\mnisttrb{} & 893K \\ 
Resnet18 & 11.1M \\ 
\midrule
\textbf{Hyperparameter} & \textbf{Value} \\ 
\midrule
Batch Size & 256 \\ 
Max Optimization Steps & 15,000 \\
Encoder Loss Update Frequency & 2 \\ 
Embedding Dimension & 128 \\ 
Temperature & 0.1 \\  
Contrastive Loss Weight & 1 \\ 
Budget & 0.3 \\ 
Generator Loss Update Frequency & 1 \\ 
Generator Learning Rate & 0.0001 \\ 
Generator Optimizer & Adam \\ 
Generator Weight Decay & 0 \\
On Manifold Loss Weight & 10 \\ 
Contrastive Loss Weight & 2 \\  
Discriminator Learning Rate & 0.0001 \\ 
\bottomrule
\end{tabularx}
\caption{Hyperparameters and the number of parameters per module used in training the \ofirmodel{} on the MNIST dataset.}
\label{tab:mnist_hyperparameters}
\end{table}

\begin{table}[h]
\centering
\begin{tabularx}{\linewidth}{Xr}
\toprule
\textbf{Module} & \textbf{\# Parameters} \\ 
\midrule
Generator & 1.8M \\
Discriminator & 1.6M \\
STN-CNN & 855K \\ 
Resnet50 & 23.6M \\ 
\midrule
\textbf{Hyperparameter} & \textbf{Value} \\ 
\midrule
Batch Size & 128 \\ 
Max Optimization Steps & 100,000 \\
Encoder Loss Update Frequency & 1 \\ 
Embedding Dimension & 350 \\ 
Temperature & 0.1 \\  
Contrastive Loss Weight & 1 \\ 
Budget & 0.015 \\ 
Generator Loss Update Frequency & 1 \\ 
Generator Learning Rate & 0.0001 \\ 
Generator Optimizer & Adam \\ 
Generator Weight Decay & 0 \\
On Manifold Loss Weight & 5 \\ 
Contrastive Loss Weight & 5 \\  
Discriminator Learning Rate & 0.0001 \\ 
\bottomrule
\end{tabularx}
\caption{Hyperparameters and the number of parameters per module used in training the \ofirmodel{} on the GTSRB dataset.}
\label{tab:traffic_hyperparameters}
\end{table}
\begin{table}[h]
\centering
\begin{tabularx}{\linewidth}{Xr}
\toprule
\textbf{Module Name} & \textbf{\# Parameters} \\ 
\midrule
Generator & 1.8M \\
Discriminator & 2.8M \\
Resnet18 & 11.3M \\ 
Resnet50 & 23.9M \\ 
Resnet50W & 67.2M \\ 
\midrule
\textbf{Hyperparameter} & \textbf{Value} \\ 
\midrule
Batch Size & 24 \\ 
Max Optimization Steps & 60,000 \\
Encoder Loss Update Frequency & 1 \\ 
Embedding Dimension & 2,048 \\ 
Temperature & 0.1 \\  
Contrastive Loss Weight & 1 \\ 
Budget & 0.025 \\ 
Generator Loss Update Frequency & 2 \\ 
Generator Learning Rate & 0.0001 \\ 
Generator Optimizer & Adam \\ 
Generator Weight Decay & 0 \\
On Manifold Loss Weight & 10 \\ 
Contrastive Loss Weight & 2 \\  
Discriminator Learning Rate & 0.0001 \\ 
\bottomrule
\end{tabularx}
\caption{Hyperparameters and the number of parameters per module used in training the \ofirmodel{} on the \birds{} dataset.}
\label{tab:birds_hyperparameters}
\end{table}


==> tables/apx_traffic_examples.tex <==

\begin{figure*}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/traffic_showcase-14.png}
  \caption{Evasion Attacks on \traffic{} dataset representative, Part 3. on the left we have the original image, then the EAs using FGSM, then the diff. on the right side, we have the same paradigm for EAs generated using \ofirmodel{} model.}
  \label{fig:traffic_showcase3}
\end{figure*}
